The Toxicity Phenomenon Across Social Media

Social media platforms have evolved rapidly in modernity without strong regulation. One clear obstacle faced by current users is that of toxicity. Toxicity on social media manifests through a number of forms, including harassment, negativity, misinformation or other means of divisiveness. In this paper, we characterize literature surrounding toxicity, formalize a definition of toxicity, propose a novel cycle of internet extremism, list current approaches to toxicity detection, outline future directions to minimize toxicity in future social media endeavors, and identify current gaps in research space. We present a novel perspective of the negative impacts of social media platforms and fill a gap in literature to help improve the future of social media platforms.

==> sections/botstrolls.tex <==
% \section{\textcolor{green}{Bots vs. Trolls}}
% \section{\textcolor{red}{Bots vs. Trolls}}
\section{Bots and Trolls}
\label{sec:botstrolls}
%Humans are no longer the only actors in online spaces. 
To understand how people are affected by toxicity 
, we must first identify and understand all the actors in the space, including bots and trolls. 
%of which bots and trolls are indisputably counted among. 
% As social media has evolved, a number of platforms (especially those with lax account creation standards such as Twitter) have cultured spaces where a single user can manage a large number of accounts. %Users can create accounts to engage with a separate community. 
% For example, a Twitter user can have one account to engage with political content and another account to engage with pop culture.
% Recently, partly due to the ease of account creation, %polarization of online discourse and 
% the practice of online "trolling" has been on the rise. %These two ideals could be contributing to flourishing practice of online 'Trolling.' 
A \textbf{troll account} has the primary objective of spreading discourse. Troll's posts and comments are incendiary and most times published with the intent to cause the most extreme reaction. 

Twitter accounts can be operated and maintained completely via API calls. As a result, humans are no longer the only users in online spaces. This account control feature in conjunction with the ease of creating multiple accounts, has allowed for a developed economy of bots to thrive. \textbf{Bot accounts} are run and managed by sophisticated software which is capable and ready to capitalize on nuanced conversations in an attempt to sway public opinion. These accounts are often members of a larger \textbf{bot swarm}, which operates towards a unified goal.

% Though bots involved in swarms often have a specific goal, not all bot %or ever bot 
% swarms have malicious intent and can be utilized to perform any number of automated tasks (such as posting weather updates%or sounding off in the event of an emergency
% ). Though the phenomena of bot and troll accounts seems inextricably tangled, it is important to remember that not all trolls are bots and vice-versa. 
Currently, even though bot profiles account for only 5\% of all Twitter profiles, it is estimated that 20-30\% of Twitter content consumed in the US is created by bots~\cite{varanasi}. 
%it is estimated that between 20-30\% of Twitter content consumed in the US is created by Bot accounts. This number is a considerable portion considering that bots account for only 5\% of all Twitter profiles~\cite{varanasi}. 
This percent disparity demonstrates how great the reach of these bot accounts. 

% Given the potential for a bot account to reach large number of people, bot creators have weaponize this opportunity in a number of ways, including: attempts to sway election results~\cite{dutta2021analyzing}, rehabilitate brand reputation~\cite{aydemir2020social}, and boost album sales~\cite{boyer_2021}. 

%This may be removed for the sake of space
Many tools have been created to identify bot accounts, but these are not easily integrated into existing SMP spaces. Tools that distinguish real users from bot accounts often appear to do so with high-accuracy, though with a tendency towards false positives when considering users with deviant behavior~\cite{rauchfleisch2020false}.  And yet, these identification tools are not integrated with existing platforms given the lack of incentives to do so for SMP operators, leaving users to operate in spaces where the autonomy of any account may be an illusion. 




==> sections/methodology.tex <==
\section{Methodology}
\label{sec:method}

==> sections/ramifications.tex <==
%@Rhett: I am leaning towards commenting out this whole section as it deters from our original intent of understand online toxicity. I am not too sure of this decision, so feel free to push back if you disagree.
% \section{\textcolor{green}{Ramifications}}
% \section{\textcolor{red}{Ramifications}}
% \section{Ramifications}
% \label{sec:ramifications}

% The impact of social media usage on its users is complex, and likely out of reach. However, much past research has been devoted to this nuanced discussion. Therefore, for the purposes of this work, our discussion focuses on the mental health of users who encounter toxicity, generally in the form of 'cyberbullying' and online sexual harassment as the majority of past research in this space has considered these issues most heavily. Of particular interest to this work are longitudinal studies which have monitored participants over a number of years and examined sustained effects.

% As has been previously established, teens and young adults on the Internet are the most affected demographic. In one multi-year longitudinal study which focused on prevalence, predictors and consequences of cyberbullying and online sexual harassment among teenagers a number of short and long term effects were observed~\cite{copp2021online}. Victims of either of these forms of toxicity (cyberbullying or online sexual harassment) were shown to report higher levels of marijuana and alcohol usage, depressive symptoms, and even physical aggression manifesting outside of virtual spaces when compared with teens who had not experienced either form of toxicity. When considering only users who reported experiencing online sexual harassment, even after controlling for past behaviors, these users were more than two times as likely to engage in marijuana and alcohol usage and exhibit physical aggression, and 1.7 times as likely to show depressive symptoms for at least two years after their reported experience. Victims of cyberbullying showed similar susceptibilities to these effects. %~\cite{copp2021online}. %Specifically, cyberbullied teens were found to be more than two times likely to partake in alcohol usage and become physically aggressive, and nearly two times as likely to use marijuana and become depressed, when compared with teenagers who did not experience cyberbullying . These effects were shown to persist across the entirety of the two-year study.

% %While generally male and female teens appear to be similarly affected by cyberbullying, female teens report using alcohol at increased rates after cyberbullying victimization, even when compared with male teens who have reported similar experiences~\cite{copp2021online}. Female teenagers who have experienced online sexual harassment as also more prone to cope with marijuana usage and depressive behaviors than their male counterparts~\cite{copp2021online}.

% %Teens who reported experiencing both forms of toxicity, online sexual harassment and cyberbullying showed exacerbated consequences~\cite{copp2021online}. In particular, these users showed increased rates of marijuana usage and depressive symptoms, again persisting even two years after their experiences with these negative online behaviors~\cite{copp2021online}. Unsurprisingly, this same work reports that teens who reported never experiencing online sexual harassment or cyberbullying showed significantly reduced rates of alcohol and marijuana usage, physical aggression and depressive symptoms~\cite{copp2021online}.

% Other work has found adolescents who encounter cyberbullying (as either the aggressor or victim) show associated increased risk of involvement with delinquent peers~\cite{guo2022cyberbullying}. Much past work has shown that such delinquent peer involvement leads to high levels of physical fighting and substance use.

% One longitudinal study, which following adults workers over a number of years in Finland, found that cyberbullying at work leads to psychological distress, `technostress' (or increased stress surround the use of technology), work exhaustion, and decreased work engagement~\cite{celuch2021longitudinal}. These results confirmed suspicions that workers experiencing cyberbullying would perform worse than their peers who did not experience online harassment. Another important takeaway from this work, is the very measurable impact that diminished productivity can have on a company. Workers burdened by online harassment put forth less effort than their seemingly happier peers.

% While understanding the full effects of toxicity online may be difficult, the negative impact that the stress of online harassment causes individuals across all ages is clear. Research has clearly shown a pipeline which pushes individuals towards deviant behavior after experiencing online toxicity. These emerging behaviors manifest different across studies, situations, and age ranges, but underscore the notion that feeling targeted by online toxicity leads to undesirable outcomes such as increased drug and alcohol abuse, lowered self-esteem, and diminished productivity. These effects simply illustrate a few of the consequences of the negative head-space internet users faced with toxicity are left to shoulder.

% Research also supports the notion that after experiencing cyberbullying, a young person may feel empowered by cyberbullying others, possibly in an attempt to relieve negative feelings of helplessness incurred during their own victimization~\cite{garaigordobil2015cyberbullying}. Through this process, a cycle of victimization and harassment continues, wherein the victim becomes a future perpetrator. This further highlights the importance in stopping online toxicity from reaching young, impressionable internet users, as this could moderate possible one-day cyberbullies from entering into this viscous sequence. 

